Time Window Temporal Logic

This paper introduces time window temporal logic (TWTL), a rich expressivity language for describing various time bounded specifications. In particular, the syntax and semantics of TWTL enable the compact representation of serial tasks, which are typically seen in robotics and control applications. This paper also discusses the relaxation of TWTL formulae with respect to deadlines of tasks. Efficient automata-based frameworks to solve synthesis, verification and learning problems are also presented. The key ingredient to the presented solution is an algorithm to translate a TWTL formula to an annotated finite state automaton that encodes all possible temporal relaxations of the specification. Case studies illustrating the expressivity of the logic and the proposed algorithms are included.

==> figures/ast.tex <==
\begin{figure}[!htb]
\centering
\begin{tikzpicture}[
    grow = right,
    state/.style={ellipse, draw=none, fill=orange, circular drop shadow,
        text centered, anchor=west, text=black, minimum width=1cm},
    leaf/.style={ellipse, draw=none, fill=cyan, circular drop shadow,
        text centered, anchor=west, text=black},
    level distance=0.4cm, growth parent anchor=east
]

\node [state] {$\cdot$} [->, sibling distance=1.5cm]
     child {
        node [state] {$[\ ]^{[1,8]}$}
        child { [->, sibling distance=1.2cm]
            node [state] {$\andltl$}
            child {
                node [leaf] {$H^3 B$}
            }
            child {
                node [state] {$[\ ]^{[0, 4]}$}
                child {
                    node [leaf] {$H^3 C$}
                }
            }
        }
     }
     child {
        node [state] {$[\ ]^{[0,2]}$}
        child{
            node [leaf] {$H^1 A$}
        }
     }
;
\end{tikzpicture}
\caption{The AST corresponding to the TWTL in Eq.~\eqref{eq:tr-example-twtl}.
Intermediate nodes are shown in orange and correspond to Boolean,
concatenation and within operators.
Leaf nodes are shown in cyan and are associated with hold operators.
}
\label{fig:ast-example}
\end{figure}
